A Survey of Large Language Model Agents for Question Answering

This paper surveys the development of large language model (LLM)-based agents for question answering (QA). Traditional agents face significant limitations, including substantial data requirements and difficulty in generalizing to new environments. LLM-based agents address these challenges by leveraging LLMs as their core reasoning engine. These agents achieve superior QA results compared to traditional QA pipelines and naive LLM QA systems by enabling interaction with external environments. We systematically review the design of LLM agents in the context of QA tasks, organizing our discussion across key stages: planning, question understanding, information retrieval, and answer generation. Additionally, this paper identifies ongoing challenges and explores future research directions to enhance the performance of LLM agent QA systems.

==> Intro/v1.tex <==
\section{Introduction}
The autonomous agent has been recognized in the long term. It can perceive the environment and autonomously act upon it, pursuing the initial set goals~\cite{franklin1996agent}. In previous studies, agents are typically trained with reinforcement learning (RL) and assumed to act following heuristic policy functions in a restricted environment~\cite{mnih2015human,lillicrap2015continuous}. Despite the achievements of these RL-based agents, they always face some significant challenges: i) training an expert agent for new scenarios requires a substantial number of samples, and incurs high costs from the expert's reward design; ii) the trained agent lacks world knowledge and fails to accommodate to the various input or the complex environment.

With the rapid development of large language models (LLMs), LLM-based agents have garnered attention~\cite{park2023generative,wang2024survey}. The LLM is a neural network-based language model, typically composed of billions or even hundreds of billions of parameters, capable of handling complex natural language tasks. By training on vast amounts of text data, LLMs can learn the grammar, semantics, context, and world knowledge of language. They excel at transforming various NLP tasks into end-to-end text generation tasks, achieving significant performance improvements across multiple tasks. LLM can be used as the ``brain'' in building an agent. Compared with the RL-based method, the LLM-based method has addressed the limitations aforementioned. First, LLM agents can capture a wide range of language patterns and have comprehensive world knowledge, enabling them to have strong generalization capabilities. When faced with new tasks or environments, they can quickly adapt with just prompting instructions or a small amount of data. Second, LLMs have shown powerful reasoning skills, handling complex questions even in the absence of direct training in specific environments. Additionally, it takes natural language as input, which is flexible, explainable, and user-friendly.

Question answering (QA) has been a traditional research direction in NLP for decades and is a widely adapted application for LLM-based agents. The definition of QA is to provide the correct answers to questions based on some given context or knowledge, aiming to fill human information needs~\cite{jm3}. It is important to note that nearly all NLP tasks can be transformed into a QA format, e.g., translation can be framed as, "\textit{Can you provide me with the translation of the following sentence?}". Therefore, in this paper, we focus only on tasks where the user has an explicit information need.

Although LLMs can directly answer the question, they still suffer from limitations. The first problem is that LLM can have hallucinations in generating the answers. LLMs may produce answers that are imprecise, or even wrong, especially when nuanced, domain-specific knowledge is required. This is particularly evident in complex tasks like legal, financial, or medical decision-making~\cite{cui2024chatlaw,financemath}. Secondly, the LLM cannot interact with the environment. It cannot interact with external databases to retrieve fresh information or tools (e.g., calculators, APIs) to get more accurate answers. On the other hand, while LLMs can generate plausible answers, they can't verify the correctness of their outputs autonomously in the environment. 

To address these issues, the LLM-based agent is proposed. The main difference between LLM-based agents and only LLM in QA tasks is that LLM-based agents are equipped with multiple heuristic-designed modules for guiding the LLM in performing specific actions, e.g., planning, reasoning, and can interact with external environments, including databases, tools, other trained models, and humans.

In this paper, we conduct a comprehensive survey of the design of LLM agents for QA. We first present the preliminary knowledge needed to understand this survey. Then we summarize the current research works about LLM agents in QA. Specifically, we first introduce the QA tasks and then organize our summary based on each stage in the QA process. We split stages in QA into planning, question understanding, information retrieving, answer generation, and follow-up interaction. For each stage, we introduce the motivation of involving agent design and how to design the LLM agent to make LLM perform better in this stage. After reviewing the current work, we identify various challenges in this field and discuss potential future directions. 

The research mentioned in this survey frequently appears in top-tier conferences and journals within the fields of NLP. Key venues for these publications include the Annual Meeting of the Association for Computational Linguistics (ACL), the Conference on Empirical Methods in Natural Language Processing (EMNLP), and the North American Chapter of the Association for Computational Linguistics (NAACL). Additionally, influential papers are often presented at AI conferences such as the International Conference on Learning Representations (ICLR) and the Conference on Neural Information Processing Systems (NeurIPS), etc. These venues are recognized for their rigorous peer-review processes and high impact in advancing research in AI and NLP.


==> Preliminary/v1.tex <==
\section{Preliminary}

\subsection{Question Answering}
Question Answering (QA) is a task where a system is designed to automatically provide answers to questions posed by users. It serves as a crucial application across multiple domains, including search engines, customer support, and education \cite{voorhees1999trec}. 

Let \( Q \) be the input question, \( C \) be the given context, and \( A = (a_1, a_2, \dots, a_T) \) be the answer sequence composed of \( T \) tokens. \( P(A | Q) \) is the probability of generating the answer given the question.
Categorized by the answer format, QA systems were generally built using three main approaches: classification-based methods, span-extraction methods, and text-generation methods. 

In the classification paradigm, given multiple possible answers $A_1$, $A_2$,..., $A_n$, the system is treated as a multi-class classifier, where each possible answer corresponds to a distinct class \cite{manning2008introduction}. It could be denoted as:
\begin{equation}
P(A_i | Q) = \text{classifier}(Q,C;\theta)
\end{equation}
where \( A_i \) is the predicted answer from the set of possible answers \( A_1, A_2, \dots, A_n \).

On the other hand, span-based methods involve identifying a span of text in a given document or context that contains the answer \cite{rajpurkar2016squad}.
\begin{equation}
P_s = \text{classifier}(C_s, Q;\theta), \quad P_e = \text{classifier}(C_e, Q;\theta)
\end{equation}
where \( C_s \) and \( C_e \) are the tokens for the start and the end position and \( P_s \) and \( P_e \) are the probabilities of the answer span in the context \( C \).

In contrast to span extraction, text generation models approach QA as a sequence generation task. Given a question, the model makes the classification token-by-token:
\begin{equation}
P(A | Q) = \prod_{t=1}^{T} P(a_t | Q,C, a_1, a_2, \dots, a_{t-1};\theta) \label{eq: text_generation}
\end{equation}
where the model generates each token \( a_t \) based on the question \( Q \), content \( C \), and the previously generated tokens \( a_1, a_2, \dots, a_{t-1} \).
Early efforts in text generation for QA include neural sequence-to-sequence models, where an encoder maps the input question to a latent representation, and a decoder generates the answer \cite{bahdanau2014neural}.
While these methods demonstrated some success in getting more nuanced answers, they struggled with long-term dependencies and accuracy, especially in open-domain settings \cite{vinyals2015pointer}.

LLM-based QA using pre-trained LLMs to understand and generate answers, often by fine-tuning them on specific datasets or prompting them in few-shot settings, has redefined QA paradigms. As a text generation method, it follows the same formula as \ref{eq: text_generation}.
Unlike traditional QA methods, LLMs can perform open-domain QA directly, leveraging their extensive knowledge encoded from large-scale pretraining \cite{petroni2019language}. 
This allows LLMs to generate coherent and contextually relevant answers, even for questions they were not explicitly trained on. 
Despite their strengths, LLM-based QA models have several limitations. 
One significant issue is the phenomenon of hallucination, where the LLM generates factually incorrect but plausible-sounding answers \cite{ji2023survey}. This occurs because the LLM does not have mechanisms to perform calibration by itself. 
Another key challenge is that LLMs cannot consult external databases, APIs, or other dynamic sources during inference \cite{lewis2020retrieval}. 
Once trained, the model's parameters are fixed, and it must rely entirely on its internalized knowledge to generate answers. 
% For example, an LLM trained on a corpus up to a specific date may fail to provide accurate answers to questions about events that occurred after its last update \cite{bommasani2021opportunities}. 
This makes it difficult for LLMs to respond accurately to queries requiring up-to-date or long-tail information, such as real-time financial data, medical knowledge, or recent research developments \cite{bommasani2021opportunities,komeili2022internetaugmented}. Additionally, even if a LLM has the relevant information in its pretraining data, retrieving and reasoning over that information at inference can be unreliable due to the model's implicit memory, which is not designed for explicit information retrieval \cite{guu2020retrieval}. Therefore, the LLM-based QA agent is designed to tackle these issues.

To overcome the limitations of standalone LLMs in QA, LLM-based agents are emerging as a superior solution. An LLM-based agent can integrate additional tools and resources, such as search engines or domain-specific APIs, to verify or supplement its answers. This hybrid approach allows the agent to dynamically interact with external environments, ensuring higher accuracy and reliability \cite{schick2023toolformer}. The agent's ability to plan and execute multi-step reasoning processes ensures that it can tackle complex, multi-faceted questions by breaking them down into manageable subtasks \cite{bubeck2023sparks}. This combination of LLM reasoning and external tool usage creates a more robust, adaptable, and reliable QA system.


\subsection{LLM-based Agent}
An agent refers to a computational entity capable of interacting with its environment to achieve specific goals. Agents perceive the environment through sensors, perform reasoning or planning actions based on these perceptions, and perform actions to interact with the environment \cite{russell2003artificial}. 
% The general framework for an agent consists of a loop of observation, decision-making, and action execution.
An agent can be mathematically described through a series of equations representing its interaction with the environment. 
The agent's perception at time $t$ is given by 
\begin{equation} P_t = f(E_t) \end{equation} 
where $f$ is the sensory processing function and $E_t$ is the environment state. 
The agent's decision-making process is represented as \begin{equation} A_t = \pi(P_t, S_t) \end{equation} 
with $\pi$ being the policy function, $S_t$ the internal state, and $A_t$ the chosen action. The environment evolves according to
\begin{equation} E_{t+1} = T(E_t, A_t) \end{equation} 
where $T$ is the transition function. The agent's internal state is updated as
\begin{equation} S_{t+1} = U(S_t, P_t, A_t) \end{equation} 
with $U$ being the update function. 

Agents were first largely designed based on heuristic-based decision systems or rule-based approaches and could only handle scenarios that were explicitly programmed into them and lacked generalization abilities \cite{nilsson1982principles}. 
Reinforcement Learning (RL) based agents introduced a paradigm shift by enabling agents to learn from interaction with their environment. 
An RL agent learns by trial and error through feedback (rewards) received from its environment. 
The agent's goal is to maximize cumulative reward over time, learning optimal policies to map states to actions in an uncertain environment. 
Popular algorithms such as Policy Gradient methods have demonstrated the power of RL in complex environments like games \cite{mnih2015human}, robotic control \cite{lillicrap2015continuous}, and autonomous systems \cite{sutton2018reinforcement}.
The equation can be denoted as:
\begin{equation}
\pi^* = \text{argmax}_\pi \mathbb{E}\left[\sum_{t=0}^{\infty} \gamma^t R_t\right]
\end{equation}
Where $\pi^*$ is the optimal policy, $\text{argmax}_\pi$ denotes finding the policy that maximizes the expected cumulative reward, $\mathbb{E}$ represents the expected value, $\sum_{t=0}^{\infty}$ is the sum from time step 0 to infinity, $\gamma$ is the discount factor that determines the importance of future rewards, and $R_t$ is the reward received at time step t. 

Despite their success, RL agents face significant challenges. 
One of the primary weaknesses is sample inefficiency, as many RL algorithms require a vast amount of interaction with the environment to converge on an optimal policy \cite{silver2016mastering}. 
Additionally, RL agents struggle with exploration in large or continuous state-action spaces \cite{bellemare2016unifying}. 
These agents often require task-specific reward engineering, making them human-labor intensive and less generalizable across tasks. 
Besides, RL agents are also prone to overfitting to specific environments and can perform poorly in out-of-distribution scenarios \cite{parisotto2015actor}.

% LLMs such as GPT \cite{brown2020language} and PaLM \cite{chowdhery2022palm} are neural networks trained on massive amounts of text data.
% These models demonstrate impressive abilities in understanding and generating human language, making inferences, and even solving tasks in domains such as reasoning, coding, and common-sense understanding.
As LLMs demonstrate impressive abilities in understanding and generating human language, researchers integrate these LLMs into an agent architecture, leveraging the extensive world knowledge and language understanding capabilities of LLMs to reason and act in a broader array of tasks. 
In an LLM-based agent, the policy function $\pi$ is essentially the LLM itself. It takes the current perception $(P_t)$ and internal state $(S_t)$ as input and outputs the chosen action $(A_t)$.
Typically, the perception $(P_t)$ can be the input of texts or images, and the internal state $(S_t)$ can be thought of as the conversation history or context window and the action $(A_t)$ is a textual command to be executed. The transition function $T$ in an LLM-based agent architecture represents how the environment changes in response to the agent's actions. The update function $U$ for an LLM agent is responsible for modifying the internal state based on new perceptions and actions.

LLM-based agents are better suited for tasks requiring flexibility, knowledge generalization, and understanding of nuanced language \cite{openai2023gpt4}. These agents can operate in natural language, making them more interpretable and user-friendly. They are capable of reasoning about actions and decisions without needing large amounts of task-specific training, allowing them to generalize across tasks more efficiently than RL-agents.
The architecture of an LLM-based agent typically involves three major components: a planner, an action execution module, and a tool integration interface. The planner formulates reasoning strategies, often by simulating multiple trajectories of action or thinking steps. The action module then executes these planned actions, either within the model’s internal capabilities (e.g., generating text, solving problems) or by using external tools (e.g., APIs, web browsers). Tools enable the LLM-based agent to augment its own reasoning by accessing databases, performing computations, or interacting with external software systems. This combination of planning and tool use gives LLM-based agents a dynamic and versatile range of applications across different domains \cite{bubeck2023sparks, schick2023toolformer}.

% \subsection{Question Answering}
% Question Answering (QA) is a task in Natural Language Processing (NLP) where a system is designed to automatically provide answers to questions posed by users. It serves as a crucial application across multiple domains, including search engines, customer support, and education \cite{voorhees1999trec}. 
% A typical QA system involves several stages to process a query efficiently. 
% The first stage is \textit{question understanding}, where the system interprets the user's intent and extracts key information such as the question type (e.g., fact-based, reasoning-based) and focus (e.g., entity, event) \cite{garg2019tanda}. This is followed by \textit{planning}, where the system determines the best strategy to answer the question, such as whether to retrieve information directly or infer an answer through reasoning \cite{yang2019xlnet}. Next comes \textit{information retrieval}, where relevant documents or passages are retrieved from a corpus or knowledge base \cite{karpukhin2020dense}. 
% In the \textit{answer generation} stage, the system either extracts a specific answer span from the retrieved text or generates a full response through natural language generation \cite{devlin2018bert}. Finally, a QA system may include \textit{follow-up interaction}, which allows users to clarify their queries or ask related follow-up questions, making the interaction more dynamic and user-centric \cite{sun2022open}. The combination of these stages ensures that the QA system can handle both simple factual queries and more complex, multi-turn dialogues.

% Traditional QA systems were generally built using two main approaches: classification-based methods and span-extraction methods. In the classification paradigm, the system is treated as a multi-class classifier, where each possible answer corresponds to a distinct class \cite{manning2008introduction}. On the other hand, span-based methods involve identifying a span of text in a given document or context that contains the answer \cite{rajpurkar2016squad}. These approaches, especially the span-extraction models, have been particularly effective in closed-book settings where answers are explicitly found within a provided text.

% In contrast to span extraction, text generation models approach QA as a sequence generation task. Given a question, the model generates an answer word-by-word or token-by-token. Early efforts in text generation for QA include neural sequence-to-sequence models, where an encoder maps the input question to a latent representation, and a decoder generates the answer \cite{bahdanau2014neural}. While these models demonstrated some success in generating more nuanced answers, they struggled with long-term dependencies and accuracy, especially in open-domain settings \cite{vinyals2015pointer}.

% LLM-based QA using pre-trained LLMs to understand and generate answers, often by fine-tuning them on specific datasets or prompting them in few-shot settings, has redefined QA paradigms. Unlike traditional QA methods, LLMs can perform open-domain QA directly, leveraging their extensive knowledge encoded from large-scale pretraining \cite{petroni2019language}. This allows LLMs to generate coherent and contextually relevant answers, even for questions they were not explicitly trained on.
% Therefore, they excel at handling a wide variety of question types, from factual queries to more complex reasoning-based ones. LLMs can also generate answers without requiring an explicit retrieval step, offering a seamless and fluid QA experience \cite{roberts2020much}. Furthermore, their pretraining on diverse datasets enables them to generalize across multiple domains with minimal task-specific training \cite{jiang2020can}. This flexibility and adaptability make LLM-based QA particularly suitable for tasks involving open-ended, creative, or knowledge-intensive questions \cite{radford2019language}. 
% Despite their strengths, LLM-based QA models have several limitations. One significant issue is the phenomenon of hallucination, where the model generates factually incorrect but plausible-sounding answers \cite{ji2023survey}. This occurs because LLMs do not have mechanisms to verify facts in real time or retrieve the latest information, as their knowledge is static and frozen at the time of pretraining. For example, an LLM trained on a corpus up to a specific date may fail to provide accurate answers to questions about events that occurred after its last update \cite{bommasani2021opportunities}.
% Another key challenge is that LLMs cannot consult external databases, APIs, or other dynamic sources during inference \cite{lewis2020retrieval}. Once trained, the model's parameters are fixed, and it must rely entirely on its internalized knowledge to generate answers. This makes it difficult for LLMs to respond accurately to queries requiring up-to-date or domain-specific information, such as real-time financial data, medical knowledge, or recent research developments \cite{komeili2022internetaugmented}. Additionally, even if a model has the relevant information in its pretraining data, retrieving and reasoning over that information at inference can be unreliable due to the model's implicit memory, which is not designed for explicit information retrieval \cite{guu2020retrieval}.

% This limitation also impacts the model’s performance in niche fields where specialized or highly technical knowledge may be required. LLMs struggle to access resources that are not part of the general corpus, such as specific medical or legal databases, which hinders their utility in professional settings where access to accurate and specialized knowledge is crucial \cite{sun2022open}. Moreover, because LLMs cannot dynamically retrieve information, they lack the ability to cross-check their outputs against real-time data or external references, increasing the risk of providing outdated or erroneous answers, especially in domains where accuracy is paramount, such as healthcare or legal advice \cite{bender2021dangers}.
% This limitation in dynamic retrieval also hinders transparency and interpretability. Unlike retrieval-based systems, which can point to the specific sources or documents from which they obtained information, LLMs generate answers based on learned representations without providing traceable evidence. This makes it difficult to verify the correctness or reliability of their outputs, contributing to a lack of trust in high-stakes applications \cite{agarwal2021open}. As LLMs continue to be deployed in more critical areas, this inability to engage in dynamic, evidence-based reasoning becomes an increasingly severe limitation.

% To overcome the limitations of standalone LLMs in QA, LLM-based agents are emerging as a superior solution. An LLM-based agent can integrate additional tools and resources, such as search engines or domain-specific APIs, to verify or supplement its answers. This hybrid approach allows the agent to dynamically interact with external environments, ensuring higher accuracy and reliability \cite{schick2023toolformer}. The agent's ability to plan and execute multi-step reasoning processes ensures that it can tackle complex, multi-faceted questions by breaking them down into manageable subtasks \cite{bubeck2023sparks}. This combination of LLM reasoning and external tool usage creates a more robust, adaptable, and reliable QA system.

% The system is trained or prompted to think about the situation, make a plan, and interact with the environment~\cite{b5, b7} to better finish the goal of answering the question.

% \MY{Skills}


==> Preliminary/v2.tex <==
\section{Preliminary}
\input{overview}
\subsection{Agent}
An agent refers to a computational entity capable of interacting with its environment to achieve specific goals. Agents perceive the observation from the environment through sensors, plan actions based on these perceptions and the agent's state, and perform actions to interact with the environment \cite{russell2003artificial}. 

In Figure~\ref{fig:overview} (A), we present the overview of the naive agent. We denote the the agent's state is $S_t$ at time $t$.
The agent's planning process is represented as \begin{equation} A_{t} = \pi_p(S_t) \end{equation}
with $\pi_p$ being the planning policy function. We denote $E$ as the sensory processing function, agent's observation $O_t$ is obtained by
\begin{equation} O_t = E(A_t) \end{equation}
The new agent state is then update by 
\begin{equation} S_{t+1} = T(S_{t},A_t, O_t) \label{eq: transition}\end{equation} 
where $T$ is the transition function for defining an agent state transitioning from one to another.

Agents were first largely designed based on heuristic-based decision systems or rule-based approaches and could only handle scenarios that were explicitly programmed into them and lacked generalization abilities \cite{nilsson1982principles}. 
Reinforcement Learning (RL) based agents introduced a paradigm shift by enabling agents to learn from interaction with their environment by trial and error through feedback (rewards) received from their environment~\cite{mnih2015human,lillicrap2015continuous}. Despite their success, RL agents face significant challenges. 
One of the primary weaknesses is \textbf{generalization}, as many RL algorithms require a vast amount of interaction with the environment to converge on an optimal policy \cite{silver2016mastering}.RL agents struggle with exploration in large state-action spaces~\cite{bellemare2016unifying}. 
These agents often require task-specific reward engineering, making them human-labor intensive and less generalizable across tasks. 
Besides, RL agents are also prone to \textbf{struggle with the complex environment} and can perform poorly in out-of-distribution scenarios \cite{parisotto2015actor}.

\subsection{Question Answering}
Question Answering (QA) is a task where a system is designed to automatically provide answers to questions posed by users. It serves as a crucial application across multiple domains, including search engines, customer support, and education \cite{voorhees1999trec}.

Let \( Q \) be the input question, \( C \) be the given context, and \( A = (a_1, a_2, \dots, a_T) \) be the answer sequence composed of \( T \) tokens. \( P(A | Q) \) is the probability of generating the answer given the question.
Categorized by the answer format, QA systems were generally built using three main approaches: classification-based methods, span-extraction methods, and text-generation methods. 

In the classification paradigm, given multiple possible answers $A_1$, $A_2$,..., $A_n$, the system is treated as a multi-class classifier, where each possible answer corresponds to a distinct class \cite{manning2008introduction}. It could be denoted as:
\begin{equation}
P(A_i | Q) = \text{classifier}(Q,C;\theta)
\end{equation}
where \( A_i \) is the predicted answer from the set of possible answers \( A_1, A_2, \dots, A_n \).

On the other hand, span-based methods involve identifying a span of text in a given document or context that contains the answer \cite{rajpurkar2016squad}.
\begin{equation}
P_s = \text{classifier}(C_s, Q, C;\theta), \quad P_e = \text{classifier}(C_e, Q, C;\theta)
\end{equation}
where \( C_s \) and \( C_e \) are the tokens of the start and the end position and \( P_s \) and \( P_e \) are the probabilities of the answer start position and end position in the context \( C \).

In contrast to span extraction, text generation models approach QA as a sequence generation task. Given a question, the model makes the classification of all tokens:
\begin{equation}
P(A | Q) = \prod_{t=1}^{T} P(a_t | Q,C, a_1, a_2, \dots, a_{t-1};\theta) \label{eq: text_generation}
\end{equation}
where the model generates each token \( a_t \) based on the question \( Q \), content \( C \), and the previously generated tokens \( a_1, a_2, \dots, a_{t-1} \).
Early efforts in text generation for QA include neural sequence-to-sequence models, where an encoder maps the input question to a latent representation, and a decoder generates the answer \cite{bahdanau2014neural}.

The traditional QA pipeline is shown in Figure~\ref{fig:overview} (B). Such systems relied on breaking down the problem-solving process into several steps, executed through a fixed pipeline. These pipelines generally included the following key stages:

The system would first begin by performing syntactic analysis and semantic understanding of the user’s query. This phase involved part-of-speech tagging, dependency parsing, intent classification, and slot extraction, etc. Next, the system would use information retrieval techniques to search for potential relevant documents or sources of answers from a pre-established database, e.g., knowledge graphs, databases, documents, etc. 
Finally, as we discussed aforementioned, the system select the most probable answer from the candidate answers or extract the answer from the context or generate the answer and presented it to the user as the final output. 

The main drawbacks of such a pipeline were: (1) each sub-module required training a specialized model, and these models lacked world knowledge, making them unable to handle out-of-domain questions; (2) the pipeline was static, unable to dynamically plan the steps based on the question; (3) for open-domain questions, a vast corpus was required for retrieval and it relies heavily on the retrievers.

As shown in Figure~\ref{fig:overview} (C), LLM-based QA using pre-trained LLMs to understand and generate answers, often by fine-tuning them on specific datasets or prompting them in few-shot settings, has redefined QA paradigms. 
The mainstream pretrained LLMs can be roughly categorized into two types: \textit{Masked} LLM and \textit{Autoregressive} LLM. \textit{Masked} LLM, such as BERT~\cite{devlin2018bert}, can be used in span extract QA tasks. In this survey, we focus more on the \textit{Autoregressive} LLM, such as GPT~\cite{openai2023gpt4}, which can be used in text generation and follows the same formula as equation~\ref{eq: text_generation}.
Unlike traditional QA systems, LLMs can (1) generate coherent and contextually relevant answers, even for questions they were not explicitly trained on; (2) perform open-domain QA directly, leveraging their extensive knowledge encoded from large-scale pretraining \cite{petroni2019language}.

Despite their strengths, LLM-based QA models have several limitations. 
One significant issue is the hallucination, where the LLM generates factually incorrect but plausible-sounding answers \cite{ji2023survey}. This occurs because the LLM does not have mechanisms to perform calibration by itself. 
Another key challenge is that LLMs cannot consult external databases, APIs, or other dynamic sources during inference \cite{lewis2020retrieval}. 
Once trained, the model's parameters are fixed, and it must rely entirely on its internalized knowledge to generate answers. 
This makes it difficult for LLMs to respond accurately to queries requiring up-to-date or long-tail information, such as real-time financial data, medical knowledge, or recent research developments \cite{bommasani2021opportunities,komeili2022internetaugmented}. Additionally, even if a LLM has the relevant information in its pretraining data, retrieving and reasoning over that information at inference can be unreliable due to the model's implicit memory, which is not designed for explicit information retrieval \cite{guu2020retrieval}.

\subsection{LLM-based Agent}
To overcome the limitations of traditional QA pipelines and naive LLM QA systems, LLM-based agents are emerging as a superior solution as shown in Figure~\ref{fig:overview} (D). 
The architecture of an LLM-based agent typically involves three components: a memory part denoted as \( M \), a planning module denoted as \( \pi_p \), and an inner-thinking module denoted as \( \pi_t \). The memory $M$ is the aggregation of all the information the agent has, including the initial question $Q$, the textual result for understanding the question, and the retrieved information, etc.
For the planning module \( \pi_p \), the input is the current memory of all the information the agent has and the goal is to make a plan of which action to take in the next turn, referring to LLM with some planning prompts. For the inner thinking module \( \pi_t \), the goal is to execute some inner thinking actions, also referring to LLM itself with some different thinking prompts. 
The environment could be the physical world, the digital world (e.g., APIs, web browsers), or even humans. 

In the QA task, at time step \( t \), we use
\( A_t \) represents the action. The action space is introduced in Figure~\ref{fig:area_taxonomy}.
Actions can be divided into two types: the first is interacting with the external environment, including information retrieval and tool use, which then obtain an observation \( O_t \), subsequently storing the observation into memory \( M \). The second type is internal thinking, which does not involve interaction with the environment but still modifies the agent's memory \( M \). 
It is important to note that whether an action is for internal reasoning or interaction with the environment depends entirely on whether the agent itself is the one performing the action, rather than the content of the action. For example, in the case of question expansion, if the agent performs this operation on its own, it counts as internal reasoning. Conversely, if the agent delegates the task to an external entity, such as asking a human to perform the question expansion, the action is considered an interaction with the environment.

\input{agent_alg}
The process is shown in the algorithm~\ref{alg:llm-agent}. We initialize the memory \( M \) with the question $Q$. For $t$ time, we get the action $A_t$ based on the planner \( \pi_p \) as \begin{equation} A_{t} = \pi_p(M) \end{equation}
If the $A_t$ within the actions for the interaction of the external environment, the $O_t$ is obtained by
\begin{equation} O_t = E(A_t) \end{equation}
where $E$ is the environment feedback function. 
Then the memory is updated as 
\begin{equation} M = M||(A_t,O_t) \end{equation}
where $||$ denotes concatenation.

If the $A_t$ within the actions for thinking, then the thought $T_t$ is obtained by 
\begin{equation} T_t = \pi_t(A_t) \end{equation}

After getting the state, memory is updated as 
\begin{equation} M = M||(A_t,T_t) \end{equation}

\subsection{Comparison between LLM-based QA agent and other approaches}
\subsubsection{LLM-based QA agent v.s. conceptual agent} 
\paragraph{Similarity} LLM-based QA agent is a special case for the conceptual agent. The planning policy network for the LLM-based agent is typically LLM itself. The agent state from the general agent is considered the memory $M$ in the LLM-based agent and the transition function $T$ in equation~\ref{eq: transition} is the concatenation. 
\paragraph{Difference and motivation to have the LLM agent} The difference is for the action, that the LLM-based agent can not only interact with the environment but also activate inner thinking. As a special case for the conceptual agent, the LLM agent shows a better generalization ability and reasoning ability than the other agents, such as RL-based agents.

\subsubsection{LLM-based QA agent v.s. traditional QA pipeline} 
\paragraph{Similarity} The main similarity between LLM-based QA agents and traditional QA pipelines is that they all break down the question-answering processes into multiple actions.
\paragraph{Difference and motivation to have the LLM agent} First, LLM-based QA agents share the same advantages as the naive LLM QA system, e.g., no need for training and easily adapted to the open-domain QA. Besides, in the traditional QA pipeline, the action trajectory is pre-defined and static while the LLM-based agent QA system has the planning part to dynamically decide the action. For example, ReAct~\cite{yao2022react} lets the LLM decide what to retrieve and is the current retrieved information is enough to answer the question, while a traditional QA system cannot dynamically decide this and can only perform static steps in retrieving.    


\subsubsection{LLM-based QA agent v.s. Naive LLM QA system}
\paragraph{Similarity} The main similarity between LLM-based QA agents and naive LLM QA system is that they share the same ``brain'' and the performance is highly influenced by the LLM's ability.
\paragraph{Difference and motivation to have the LLM agent} Although LLMs demonstrate impressive abilities in QA tasks, an agent architecture would further improve the QA performance. An LLM-based agent can integrate additional tools and resources, such as search engines or domain-specific APIs, to verify or supplement its answers. This hybrid approach allows the agent to dynamically interact with external environments, ensuring higher accuracy and reliability \cite{schick2023toolformer}. The agent's ability to plan and execute multi-step reasoning processes ensures that it can tackle complex, multi-faceted questions by breaking them down into manageable subtasks \cite{bubeck2023sparks}. This combination of LLM reasoning and external tool usage creates a more robust, adaptable, and reliable QA system.

==> Taxonomy/v1.tex <==
\section{Area Taxonomy}
A typical QA system involves several stages to process a query efficiently.
\textit{Planning} is the inner ability of the LLM agent where the system determines the best strategy to answer the question, such as how to understand the query, whether to retrieve information directly or infer an answer through reasoning, etc.

% The first stage is \textit{question understanding}, where the system interprets the user's intent and extracts key information such as the question type (e.g., fact-based, reasoning-based) and focus (e.g., entity, event) \cite{garg2019tanda}. Next comes \textit{information retrieval}, where relevant documents or passages are retrieved from a corpus or knowledge base \cite{karpukhin2020dense}. 
% In the \textit{answer generation} stage, the system either extracts a specific answer span from the retrieved text or generates a full response through natural language generation \cite{devlin2018bert}. 
Besides, a QA system may include \textit{follow-up interaction}, which allows users to clarify their queries or ask related follow-up questions, making the interaction more dynamic and user-centric \cite{sun2022open}.
The combination of these stages ensures that the QA system can handle both simple factual queries and more complex, multi-turn dialogues. 


\section{Taxonomy-based Survey}
\input{taxnomy}
\subsection{Datasets}
The emergence of LLMs has led to significant advancements in question-answering (QA) tasks, necessitating the development of diverse and challenging datasets. These datasets can be broadly categorized into closed-domain/context-based QA and open-domain QA. Closed-domain QA datasets often focus on reading comprehension, such as DROP \cite{drop} and HotpotQA \cite{hotpotqa}, or knowledge-intensive tasks like FinQA \cite{financemath} and LawBench \cite{lawbench}. Open-domain QA datasets, which do not provide explicit references. It includes factual QA datasets like StrategyQA \cite{strategyqa}, ASQA \cite{asqa}, and ELI5 \cite{eli5}, mathematical reasoning datasets such as GSM8k \cite{gsm8k}, MATH \cite{math}, DeepMind Math \cite{deepmindmath}, Olympic Math \cite{olympicmath}, symbolic reasoning datasets, such as BBH \cite{bbh} and Folio \cite{folio}, and knowledge-intensive reasoning datasets through MMLU \cite{mmlu}, GPQA \cite{gpqa}, and WikiQA \cite{wikiqa}. Besides, the conditional reasoning is explored in datasets like IFQA \cite{ifqa}. 
The diverse nature of these datasets allows for comprehensive evaluation of LLMs across various dimensions of QA tasks.

\subsection{Planning}
The \textit{planning} aspect is crucial in enhancing the reasoning process during QA tasks and is the key to making the agent \textbf{autonomous}. Planning refers to the mechanism by which an agent decides on a series of intermediate steps or actions to reach a final answer to a given query. There are two primary paradigms in planning:
% \paragraph{Planning with Manually Pre-defined Rule} The manually predefined planning paradigm provides explicit rules or strategies for the LLM to follow, helping it follow structured pathways for complex problem-solving.

% Many works aim to improve performance through manually predefined workflows, e.g., the LLM is first prompted to decompose the question and then solve it, recall relevant information from a database before solving, or validate the solution after completion, etc.

% In these cases, each step is predetermined and cannot be skipped. This approach is primarily suited for scenarios where the source of the questions is relatively uniform, and a static workflow can handle the vast majority of problems.
 
\paragraph{Tuning-free planning} LLM is prompted by well-formulated prompts, thus leveraging the LLM's latent knowledge for decision-making of action. \cite{sun2023think, zhou2023solving,yao2022react,jiang2023active} design a heuristic prompt to leverage the LLM to decide if the current information is enough to answer the question. \cite{chen2023agentverse} prompts the LLM to select the best expert models/agents to find the information. \cite{gao2023enabling, yao2022react} also prompt LLM to decide if the problem-solving processing should be posted to the next stage.
\paragraph{Tuning-based planning} It involves iterating over incorrect trajectories and refining strategies through trial and error, ultimately improving the LLM's reasoning capabilities by learning optimal paths from past mistakes. FireAct~\cite{chen2023fireact} fine-tuned the LLM by agent trajectories generated from multiple
tasks and unified in the ReAct~\cite{yao2022react} format. Learning From Failure\cite{wang2024learning} leverages the LLM to learn from the comparison of successful and failed trajectories. AgentGen\cite{hu2024agentgen} focuses on generating planning tasks conditioned on these environments and then finetuning the planner with the synthesized data.


\subsection{Question Understanding}
The question-understanding process requires extracting and comprehending information from the user’s query and making it easier for the machine to understand. Users' questions can be ambiguous or complex, so multiple techniques are used to help the machine process the question to make the answer easier.
Traditionally, separate models were trained specifically for tasks like slot tagging and intent understanding~\cite{chen2019ICSF}. 
As LLMs show the inherent ability to handle complex linguistic structures, the research made them useful for performing question understanding without the need for task-specific models.
\paragraph{Identifying Slots}
Identifying slots refers to the process where specific entities, variables, or attributes within a query are recognized and categorized based on predefined types or structures. 
% These slots often represent the essential pieces of information required to complete or fulfill a query in tasks such as dialogue systems, information extraction, or structured database querying \cite{mesnil2015}. 
The motivation is to bridge unstructured natural language input with structured data representations, enabling more precise and context-aware responses. 
% By accurately detecting and categorizing slots (e.g., locations, dates, or item types), systems can better tailor responses, improving performance in tasks like task-oriented dialogue and question answering \cite{zhang2019}. 
% Moreover, slot identification plays a crucial role in modularizing the processing pipeline, allowing different parts of the system to handle specific aspects of the query in a structured way.
In LLM-based agent applications, Chatlaw\cite{cui2024chatlaw} selects appropriate law-related entity clusters based on the consultation question in identifying slots by prompting LLM with the context.

\paragraph{Query Expansion}
Query expansion enhances the retrieval of relevant information by adding additional terms or phrases to the original query. This can include synonyms, related concepts, or more specific details based on the context of the search or question \cite{carpineto2012}.
A user's initial query might be too vague, ambiguous, or incomplete to retrieve the best possible results. By expanding the query with terms that are semantically related, systems can increase recall, improving the chance of retrieving documents or passages that match the user's intent \cite{robertson2004}.
% Query expansion is especially beneficial in information retrieval and question answering systems, where the accuracy and relevance of the retrieved content are directly tied to the quality and completeness of the query formulation.
In the LLM-agent QA system, query expansion is especially popular and beneficial as LLMs possess extensive world knowledge and strong associative capabilities, which are highly beneficial for question expansion. 
HyQE~\cite{gao-etal-2023-hyqe} prompts the LLM to generate multiple hypothetical documents as the expansion of questions. 
Query2cot~\cite{jagerman2023querycot} prompts instruct the LLM to break the questions down step-by-step and make the LLM think about the keywords for each question.

\paragraph{Query Reformulation}
Query reformulation refers to rephrasing or simplifying the original query to address issues such as ambiguity, vagueness, or overly broad formulations in the user's original input. RR~\cite{deng2023rephrase} prompts the LLM to rewrite the question to a better one and \cite{ma2023query, Peng2023Taobao} trains the LLM specified to rewrite the query. Step-back reformulation~\cite{zheng2023takestepback} first reformulate the original reasoning questions into their high-level concept questions and then use LLM to answer these high-level questions aiding the original questions. 
% This modification can include rephrasing, simplifying, or adding context to the query. 
% The motivation behind query reformulation is to address issues such as ambiguity, vagueness, or overly broad formulations in the user's original input. 
% By refining the query, systems can better align the user's intent with the underlying information sources, thereby improving retrieval precision and user satisfaction. 
% Query reformulation is particularly useful in information retrieval, search engines, and question answering systems, where slight modifications to the query can significantly affect the relevance and quality of the retrieved results.
% Additionally, it plays a critical role in systems that handle conversational or complex multi-turn interactions, allowing the system to progressively refine and better understand the user's needs.






\subsection{Information Retrieval}
The \textit{information retrieval} component in LLM-based QA agents is pivotal in answering knowledge-intensive questions for extracting relevant knowledge from a vast corpus or external knowledge sources. Information retrieval refers to the process of identifying and ranking documents, passages, or snippets that may contain the necessary information to answer a given question. This process generally follows a \textbf{retrieving-and-ranking} paradigm, involving several techniques. 
\paragraph{Retrieval} The initial step, retrieval, involves fetching a set of candidate documents or passages using sparse or dense retrieval techniques. 
Sparse retrieval methods, such as BM25~\cite{jm3}, rely on term frequency-inverse document frequency (TF-IDF) based ranking algorithms. However, sparse methods often struggle with semantic mismatches where the query and document might have a similar meaning but use different terms.

Dense retrieval relies on learning vector representations for both the query and documents, embedding them into a shared semantic space where the relevance between them can be measured via similarity scores.
Once the query $q$ and document $d$ are embedded into vectors, we compute the similarity between the two using a distance metric, often cosine similarity: \begin{equation} sim(q, d) = \frac{q \cdot d}{|q| |d|} \end{equation}
A commonly employed dense retrieval model is based on the contrastive learning objective, where the goal is to maximize the similarity between a query and a relevant (positive) document while minimizing the similarity with irrelevant (negative) documents. This can be represented mathematically through the loss function: 
\begin{equation}
\mathcal{L} = \log \frac{e^{sim(q_i, d_i^+)}}{e^{sim(q_i, d_i^+)} + \sum_{j=1}^{N} e^{sim(q_i, d_j^-)}}
\end{equation}
where $d_i^+$
is the positive sample of the query, and $d_i^-$ is the negative one. N is the number of negative samples~\cite{gao2024modular}. The similarity function $sim(q_i, d)$, often implemented as the dot product or cosine similarity of the embeddings, is designed to capture the closeness between the query and document representations.

\paragraph{Ranking} This is followed by retrieving, where an additional model, such as a trained neural network, assigns scores to the retrieved candidates, refining their relevance. Haystack~\cite{ranker} leverages the LLM to decide the relevance score of retrieved candidates. \cite{ma2023large,zhuang2023open} indicate that LLM is not good at retrieving but good at re-ranking the hard examples.

\paragraph{Compression and Selection}
Excessive context can
introduce more noise, diminishing the LLM’s perception of
key information. Ranking methods also include compression and selection, which summarizes or distills long documents to focus on essential information, and selection, where specific passages are chosen to be forwarded to the reasoning model based on their relevance scores. 
The integration of these steps enhances the ability of the LLM to answer questions accurately by narrowing down and selecting the most pertinent information from the retrieved set.
LLMLingua ~\cite{jiang2023longllmlingua} is proposed to compress the information in the prompt towards improving LLMs' perception of the key information. PRCA~\cite{yang2023prca} and Rrecomp~\cite{xu2023recomp} are to fine-tune the LLM for the key information extraction. \cite{ma2023large} propose to first select the most relevant document and filter the irrelevant ones.

\subsection{Answer Generation}
The answer generation component in LLM-based QA agents is to make the model synthesize relevant information and output the answer to the given query as the formula~\ref{eq:text_generation}. This process can follow multiple methods in boosting answer generation in LLM-based agents.

\paragraph{Tool-augmented Generation} LLM can interact with the environment and leverage external tools, such as calculators, code interpreters, or external APIs, to augment its reasoning capabilities and improve precision in tasks requiring specialized knowledge. PoT~\cite{chen2022pot,gao2023pal} uses the LLM to write the Python code and uses the interpreter to execute the code and get the final answer. HuggingGPT~\cite{shen2024hugginggpt} and Openagi~\cite{ge2024openagi} take the other domain-specific models, such as the image segmentation model, as external tools for providing information that LLM may hard to know. \cite{cheng2022binding, gao2024efficient} prompt the LLM to generate the skeleton of the answer and use external tools, such as a calculator or code interpreter, to make the answer precise. 

\paragraph{Prompt-Enhanced Generation} Various prompting engineering methods can be employed to improve the answer-generation process in LLMs. The prompt can be designed by heuristic design or automatically generated. The CoT approach~\cite{wei2022chain} significantly improves performance on reasoning problems by prompting LLMs to think step-by-step, thereby activating their
inherent reasoning capabilities. Advanced prompt engineering methods, such as question decomposition~\cite{zhou2023leasttomostpromptingenablescomplex} and
self-verification~\cite{chen2023teaching}, have also proven effective in improving reasoning performance. Additionally, recent approaches have incorporated automatic prompt optimization based on
training data. Self-discovery~\cite {zhou2024self-discover} utilizes modular reasoning components to construct the task-adaptive prompt. PromptAgent~\cite{wang2023promptagent} taking the prompting optimization with Monte-Carlo Tree Search.


\subsection{Follow-up Interaction}
In LLM-based QA agents, follow-up interaction plays a crucial role in maintaining engagement and ensuring clarity during the conversational flow. Unlike traditional QA systems that terminate interaction after a single response, LLM agents are naturally designed to engage in multi-turn conversations, refining their answers or asking for clarification if needed~\cite{wang2023mint}. This dynamic interaction allows the model to adapt its responses based on user feedback or changing context, improving the relevance and depth of its answers over time.

\paragraph{Error Resolution} In many instances, the initial answer generated by the LLM might not fully address the user's intent, or ambiguities in the query might lead to incomplete or incorrect responses. Follow-up interaction provides an opportunity for the model to clarify misunderstandings or ask for additional details. By prompting users with follow-up questions or offering multiple interpretations of a query, the agent can improve the accuracy of its subsequent answers. \cite{schick2022peer} explore the use of human feedback to revise the sentences and \cite{yan2023learning} use human feedback to revise the semantic parsing results. Mint~\cite{wang2023mint} explores the LLM ability to learn from human feedback.


\paragraph{Sequential Question Answering} Sequential Question Answering is to engage humans in having a follow-up interaction that involves maintaining context across multiple exchanges~\cite{iyyer2017search}. The LLM needs to track previous interactions to generate coherent responses, especially in cases where the user asks related or follow-up questions.  
In the previous studies, sequential QA requires training an extra model. However, since LLMs can engage in multi-turn conversations easily after instruction tuning and reinforcement learning from human feedback~\cite{ouyang2022training}, it is considered a naive ability for the current LLM agent. to better answer follow-up questions, ChatQA~\cite{liu2024chatqa} fine-tune the LLM with context-enhanced instruction tuning.

==> reference.tex <==
\begin{thebibliography}{00}
\bibitem{b1} Franklin, Stan, and Art Graesser. "Is it an Agent, or just a Program?: A Taxonomy for Autonomous Agents." International workshop on agent theories, architectures, and languages. Berlin, Heidelberg: Springer Berlin Heidelberg, 1996.
\bibitem{b2} Park, Joon Sung, et al. "Generative agents: Interactive simulacra of human behavior." Proceedings of the 36th annual acm symposium on user interface software and technology. 2023.
\bibitem{b3} Wang, Lei, et al. "A survey on large language model based autonomous agents." Frontiers of Computer Science 18.6 (2024): 186345.
\bibitem{survey} Cheng, Yuheng, et al. "Exploring large language model based intelligent agents: Definitions, methods, and prospects." arXiv preprint arXiv:2401.03428 (2024).
\bibitem{b4} Rogers, Anna, Matt Gardner, and Isabelle Augenstein. "Qa dataset explosion: A taxonomy of nlp resources for question answering and reading comprehension." ACM Computing Surveys 55.10 (2023): 1-45.
\bibitem{Kamalloo} Kamalloo, Ehsan, et al. "Evaluating Open-Domain Question Answering in the Era of Large Language Models." Proceedings of the 61st Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers). Association for Computational Linguistics, 2023.
\bibitem{open-domain} Li, Junlong, et al. "Self-Prompting Large Language Models for Zero-Shot Open-Domain QA." Proceedings of the 2024 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies (Volume 1: Long Papers). Association for Computational Linguistics, 2024.
\bibitem{b6} Wei, Jason, et al. "Chain-of-thought prompting elicits reasoning in large language models." Advances in neural information processing systems 35 (2022): 24824-24837.
\bibitem{b5} Yao, Shunyu, et al. "React: Synergizing reasoning and acting in language models." The Eleventh International Conference on Learning Representations. 2023.
\bibitem{reflect} Shinn, Noah, et al. "Reflexion: Language agents with verbal reinforcement learning." Advances in Neural Information Processing Systems 36 (2024).
\bibitem{b7} Gao, Luyu, et al. "Pal: Program-aided language models." International Conference on Machine Learning. PMLR, 2023.
\bibitem{b9} Shen, Yongliang, et al. "Hugginggpt: Solving ai tasks with chatgpt and its friends in hugging face." Advances in Neural Information Processing Systems 36 (2024).
\bibitem{b10} Yao, Shunyu, et al. "Tree of thoughts: Deliberate problem solving with large language models." Advances in Neural Information Processing Systems 36 (2024).
\bibitem{b11} Patil, Shishir G., et al. "Gorilla: Large language model connected with massive apis." arXiv preprint arXiv:2305.15334 (2023).
\bibitem{b12} Song, Yifan, et al. "Trial and error: Exploration-based trajectory optimization for llm agents." arXiv preprint arXiv:2403.02502 (2024).
\bibitem{b13} Schick, Timo, et al. "Toolformer: Language models can teach themselves to use tools." Advances in Neural Information Processing Systems 36 (2024).
\bibitem{b14} Zhao, Andrew, et al. "Expel: Llm agents are experiential learners." Proceedings of the AAAI Conference on Artificial Intelligence. Vol. 38. No. 17. 2024.
\bibitem{b15} Xiao Liu, et al. "AgentBench: Evaluating LLMs as Agents." The Twelfth International Conference on Learning Representations. 2024.
\bibitem{toolqa} Zhuang, Yuchen, et al. "Toolqa: A dataset for llm question answering with external tools." Advances in Neural Information Processing Systems 36 (2024).
\bibitem{rag survey} Gao, Yunfan, et al. "Retrieval-augmented generation for large language models: A survey." arXiv preprint arXiv:2312.10997 (2023).


\end{thebibliography}
\vspace{12pt}
\color{red}
